Best Buddies Registration for Point Clouds

We propose new, and robust, loss functions for the point cloud registration problem. Our loss functions are inspired by the Best Buddies Similarity (BBS) measure that counts the number of mutual nearest neighbors between two point sets. This measure has been shown to be robust to outliers and missing data in the case of template matching for images. We present several algorithms, collectively named Best Buddy Registration (BBR), where each algorithm consists of optimizing one of these loss functions with Adam gradient descent. The loss functions differ in several ways, including the distance function used (point-to-point vs. point-to-plane), and how the BBS measure is combined with the actual distances between pairs of points. Experiments on various data sets, both synthetic and real, demonstrate the effectiveness of the BBR algorithms, showing that they are quite robust to noise, outliers, and distractors, and cope well with extremely sparse point clouds. One variant, BBR-F, achieves state-of-the-art accuracy in the registration of automotive lidar scans taken up to several seconds apart, from the KITTI and Apollo-Southbay datasets.

==> OLD_00_abstract.tex <==


We propose a new loss function for the Point Cloud Registration problem. The loss is based on the Best Buddies Similarity (BBS) measure that counts the number of mutual nearest neighbors between two point clouds. This measure was shown to be robust to outliers and missing data in the case of template matching for images. However, BBS is not differentiable, because it involves a nearest neighbor search, which we overcome by using a differentiable approximation that is based on a soft argmin operator. This allows us to perform gradient descent by simply using existing neural network optimization tools. Crucially, the BBS-based loss drives the optimization while handling outliers and missing data. As a result, no pre- or post-registration steps are required. Experiments on various data sets, both synthetic and real, reveal that our algorithm is robust, accurate and enjoys a large basin of convergence.

% We propose a new loss function for the Iterative Closest Point (ICP) algorithm. The loss is based on the Best Buddies Similarity (BBS) measure that counts the number of mutual nearest neighbors between two point clouds. This loss was shown to be robust to outliers and missing data in the case of template matching for images. However, BBS is not differentiable, because it involves a nearest neighbor search, \st{and we use} \InlineAmnon{which we overcome by using a} a differentiable approximation that is based on a soft argmax operator. \st{This lets use standard neural network architecture to solve for ICP} \InlineAmnon{This allows us to perform gradient descent, which we implement as a Neural Network}. Experiments on various data sets, both synthetic and real, reveal that our algorithm is robust, \st{converges quickly} \Amnon{Our algorithm is quite slow compared to the competition. I don't think we should advertise speed. But I would write "accurate"} and enjoys a large basin of convergence.

==> OLD_01_Introduction.tex <==
\section{Introduction}



\begin{figure}
    \centering
    \includegraphics[width=1.5cm]{BBP_0.png}
    \includegraphics[width=1.5cm]{BBP_1.png}
    \includegraphics[width=1.5cm]{BBP_3.png}
    \includegraphics[width=1.5cm]{BBP_80.png}
    \includegraphics[width=1.5cm]{BBP_final.png}
     \caption{{\bf Best-Buddies Pairs:} The BBR methods perform point cloud registration by iteratively optimizing (with gradient descent) a loss defined by a set of soft or hard \emph{best buddy pairs}. Blue and Green point clouds denote the original point clouds to register. Best buddy pairs are marked in purple. From left to right: iteration 1, 2, 4, 80 and the last iteration (120). } 
     \label{fig:best_buddy_pairs}
\end{figure}


Point clouds registration is an important task in 3D computer vision. The same object or scene is scanned from two view points, e.g. with a laser scanner, and the goal is to recover the rigid transformation (rotation and translation) that aligns the two scans to each other. Realistic scenarios add complications: measurement noise, occlusions due to the change in view point, and outliers due to independent motions of free moving objects in the scene (\emph{distractors}). This makes robustness a central issue for point cloud registration algorithms. 

Probably the most popular approach to solve the problem is using some variant of the Iterative Closest Point (ICP) algorithm \cite{ICP}. This method works by iterating between two stages: first match pairs of points between the two clouds, and then apply the transformation that minimizes a loss defined by the distance between the two points in each pair. The simplest version of ICP uses the Euclidean distance between points, but later versions make use of more complex distance measures to achieve faster and more accurate convergence. %,with a larger basin of convergence.
Some of the most popular and successful variants use local normals to define point-to-plane distance measures. ICP-like methods are typically sensitive to noise, requiring the use of steps such as explicit outlier removal to improve their robustness.  

Recently, Oron {\em et al.} introduced the Best-Buddies Similarity (BBS) measure~\cite{BBS}. BBS counts the number of mutual nearest-neighbors between two point sets. This simple measure was used for template matching between images and proved to be resilient to outliers and occluders. This success motivated us to study how the BBS measure could be adapted to the task of point cloud registration. We suggest several differentiable loss functions inspired by BBS. Our registration algorithms consist of optimizing over these losses with a variant of gradient descent (Adam~\cite{articleAdam}), to recover the parameters of the aligning transformation. We collectively name the resulting algorithms \emph{Best Buddy Registration (BBR)}, and demonstrate their high level of robustness to noise, occlusions and distractors, as well as an ability to cope with extremely sparse point clouds. %Some of the algorithms also have a wide basin of convergence, and 
Some of the algorithms are able to achieve very high accuracy in noisy settings where robustness is essential. 

Deep neural networks (DNN) have increasingly been used for the processing of point clouds lately. BBR can easily be integrated into such DNNs as a registration stage, and be optimized as part of the overall gradient descent optimization of the network. To facilitate this, we implemented BBR in Pytorch, which also makes it possible to run the algorithms on widely available neural network infrastructure, such as GPUs. (See diagram in supplementary material). 

We shall now describe the different loss functions that we have defined. Our first approach was to try and use the BBS measure itself. Initial tests showed that when two point clouds are aligned, the BBS measure between them is higher than when they are not aligned. However, gradient ascent cannot be applied to the BBS measure, since it relies on a non-differentiable nearest-neighbor search. We solve this problem by making use of a soft, differentiable approximation to the nearest neighbors operation, recently suggested by Pl\"{o}tz and Roth \cite{plotz2018neural}. We name the resulting loss function \emph{softBBS}, and the registration algorithm based on optimizing it \emph{BBR-softBBS}. Though we make no use of outlier rejection, the resulting algorithm is quite robust. 


%to noise and outliers, and has a large basin of convergence. \\
We next define a second loss function which includes, in addition to the soft best-buddy scores, also the actual distances between the two points in each pair (as done in ICP). We call this loss \emph{soft buddy distance (softBD)}. The \emph{BBR-softBD} algorithm is able to achieve very high accuracy in challenging noisy scenarios. 


Both \emph{softBBS} and \emph{softBD} were defined using the simple Euclidean distance between points. A further improvement in accuracy was achieved by incorporating local normals to define a point-to-plane distance, resulting in the \emph{softBD with normals (softBDN)} loss. 

At the heart of the BBS measure lies the robustness achieved by using mutual nearest neighbors. Our final algorithm, \emph{BBR-F} is similar to existing ICP-like algorithm (such as generalized ICP~\cite{SegalHT09}, and symmetric ICP~\cite{Rusinkiewicz:2019:ASO}), except it replaces the explicit outlier rejection step with \emph{best-buddy filtering}, which is repeatedly applied at each iteration of the optimization process. This means that in the step of matching pairs between the two clouds, we only keep pairs that are mutual nearest neighbors. We demonstrate that \emph{BBR-F} is able to achieve state of the art accuracy in challenges where robustness is essential, such as registration of automotive lidar scans taken up to several seconds apart. In addition, best buddy filtering has no parameters to calibrate, unlike explicit outlier rejection. 

\iffalse
Point clouds registration is an important task in 3D computer vision. Given two scans of the same object from different locations, the goal is to find the transformation that aligns the two scans to each other. Probably the most popular approach to solve the problem is using some variant of the Iterative Closest Point (ICP) algorithm \cite{ICP}. This method matches points across the two point clouds and based on the matches minimizes some loss function. The process repeats itself until converging to a local minimum. For ICP to work well in practice, it must handle noise and converge quickly from a large basin of convergence. These goals are often supported by a judicious choice of the loss function. The standard loss minimizes the Euclidean distance between the point clouds, given the point matches, but many other options are possible. One direction is to extend the matches to be point-to-plane or plane-to-plane, that might offer fast and accurate convergence. Another direction is to robustify the loss function to deal with various types of noise such as measurement noise, distractors, and partial overlap.
\fi

\iffalse
Recently, Oron {\em et al.} introduced the Best-Buddies Similarity (BBS) measure~\cite{BBS}. BBS counts the number of mutual nearest-neighbors between two point sets. This simple measure was used for template matching between images and proved to be resilient to outliers and occluders. However, BBS is non-differentiable as it involves a nearest-neighbor search.

This work introduces a differentiable approximation to the BBS loss, and to this end, relies on the recently introduced Neural Nearest Neighbors Network of Pl\"{o}tz and Roth \cite{plotz2018neural} who proposed a soft, differentiable approximation to the nearest neighbors operation. 
Specifically, we introduce two differentiable approximations of the BBS loss function, termed {\em soft BBS loss} and {\em soft Buddy Distance loss}, and analyze their behaviour. We find that the first enjoys a very large basin of convergence, while the other is very accurate. Combining the two leads to a robust and accurate algorithm with a large basin of convergence. We further show that we can augment our loss functions with the normals of the points, if they are available, to improve accuracy. 

The proposed loss functions can be optimized by using any standard optimization tool. In this work, we chose to implement these losses in a neural network framework. Unlike a typical use of neural networks, our algorithm does not learn from a training set. Instead, it accepts a pair of point clouds as input, and the "training" is equivalent to running gradient descent optimization to find the optimal transformation between them (see Figure~\ref{fig:network_diagram}). Implementing the problem in this way has two benefits: first, it allows us to make use of neural net infrastructures that have become ubiquitous. Second, it makes it possible for the algorithm to be integrated into larger neural nets, which need to perform point clouds registration as part of their overall task. 


Experiments show that our algorithm can handle outliers, measurement noise, and partial overlap. Unlike ICP methods, it does not require any pre- or post-processing steps to achieve this robustness. It is also accurate and has a very large basin of convergence. We demonstrate its effectiveness on various cases including the challenging noisy partial shape registration problem.
\fi
% With the rise of Neural Networks, there is also a drive to embed 3D point registration into a network. Putting ICP in a neural network is difficult because a network requires the entire process to be differentiable. Yet, the matching step in ICP is non-differentiable.

% Our goal is to develop a robust neural point cloud registration algorithm that converges quickly from a large basin of convergence.  Deploying such an algorithm can take advantage of the wide deployment of neural networks across devices. Such an algorithm can also be used as a layer in neural networks.


% One of the core advantages of the proposed algorithm is that it inherits the robustness of the best-buddy similarity measure, while being differentiable at the same time, which makes it very appealing for registration. We demonstrate its effectiveness on various cases including the challenging noisy partial shape registration problem and ego-vehicle motion calculation on the KITTI dataset.

%To this end, we rely on the recently introduced Neural Nearest Neighbor Network of Pl\"{o}tz and Roth \cite{plotz2018neural} who proposed a soft, and differentiable approximation to the nearest neighbor operation. Combining the two, we are able to introduce a BBS-based loss. 

% Extensive experiments on various synthetic and real-world data sets show that the proposed algorithm has a large basin of convergence, fast convergence rate, and robustness to various types of noise.


% Many techniques have been developed for 3D registration. In general, there are three main important components in the development of such algorithms: the metric used to measure the distance between the pair of shapes, the optimization technique employed to make the shapes close to each other in this metric, and the features extracted from each shape for performing the matching. 

% Almost any registration approach can be defined by these three elements: Given two shapes, the selected optimization is performed to minimize the metric between the features extracted from them. Clearly, the underlying assumption in this generic scheme is that the metric, which serves as a loss function, is differentiable. In this work we focus on the selection of this optimization objective (the metric). 

% An important property of a loss function is that it will cause the optimization to converge towards the correct transformation, especially in the presence of large rotations and translations between two given shapes. 
% Many differentiable metric functions have been used for registration such as ... \rg{RG: A short paragraph should be added here that briefly mention the existing strategies.} Yet, their main disadvantage is their robustness to noise, outliers and partial shapes. These phenomena are very common in real object scanning and also in driving scenarios, where objects may move between two scenes. 



% A popular metric that is robust to outliers is the best-buddy similarity. It has been shown to provide high similarity between a partial object to its full shape and to be resistant to outliers. Yet, its disadvantage is that it is non-differentiable.

% This work suggests a novel approximation for the best-buddy measure that allows using it as a loss function for shape registration. We show empirically that its minimization indeed leads to the correct transformation. More specifically, its gradients point in the direction of the correct transformation, thus, allowing the use of simple gradient descent with it in the optimization. 

% One of the core advantages of the proposed framework is that it inherits the robustness of the best-buddy similarity metric, while being differentiable at the same time, which makes it very appealing for the registration task. We demonstrate its effectiveness on various cases including the challenging noisy partial shape registration problem and ego-vehicle motion calculation on the KITTI dataset.


% \begin{figure*}[!htbp]
% \label{fig:DBBR}
% 	\centering
% 	\includegraphics{network_diagram.png}
% 	\caption{Architecture of the Best-Buddy Registration network. The network takes point clouds $P$ and $Q$ as input and estimates rotation matrix $R$ and translation vector $t$. }
% 	\label{fig:network_diagram}
% 	\vspace{-0.4cm}
% \end{figure*}


% Point cloud registration is an important problem in 3D computer vision. Given two scans of the same object from different locations, the goal is to find the transformation that aligns the two scans to each other. 
% This task appears in various applications such as Odometry \cite{Geiger:2012:WRA:2354409.2354978}, and 3D object scanning and matching. 

% Many techniques have been developed for 3D registration. In general, there are three main important components in the development of such algorithms: the metric used to measure the distance between the pair of shapes, the optimization technique employed to make the shapes close to each other in this metric, and the features extracted from each shape for performing the matching. 

% Almost any registration approach can be defined by these three elements: Given two shapes, the selected optimization is performed to minimize the metric between the features extracted from them. Clearly, the underlying assumption in this generic scheme is that the metric, which serves as a loss function, is differentiable. In this work we focus on the selection of this optimization objective (the metric). 

% An important property of a loss function is that it will cause the optimization to converge towards the correct transformation, especially in the presence of large rotations and translations between two given shapes. 
% Many differentiable metric functions have been used for registration such as ... \rg{RG: A short paragraph should be added here that briefly mention the existing strategies.} Yet, their main disadvantage is their robustness to noise, outliers and partial shapes. These phenomena are very common in real object scanning and also in driving scenarios, where objects may move between two scenes. 



% A popular metric that is robust to outliers is the best-buddy similarity. It has been shown to provide high similarity between a partial object to its full shape and to be resistant to outliers. Yet, its disadvantage is that it is non-differentiable.

% This work suggests a novel approximation for the best-buddy measure that allows using it as a loss function for shape registration. We show empirically that its minimization indeed leads to the correct transformation. More specifically, its gradients point in the direction of the correct transformation, thus, allowing the use of simple gradient descent with it in the optimization. 

% One of the core advantages of the proposed framework is that it inherits the robustness of the best-buddy similarity metric, while being differentiable at the same time, which makes it very appealing for the registration task. We demonstrate its effectiveness on various cases including the challenging noisy partial shape registration problem and ego-vehicle motion calculation on the KITTI dataset.




==> OLD_04_experiments.tex <==
\section{Experiments}
\label{sec:exp}

We present experiments that are designed to analyze the behaviour of the algorithm, and evaluate it on the Stanford dataset~\cite{Turk:1994:ZPM}, as well as the TUM RGBD dataset \cite{DBLP:conf/iros/SturmEEBC12}. We then compare our approach to several established alternatives. As discussed above, we compare only to classic approaches (e.g., ICP) and not to deep network based solutions as the latter do not necessarily generalize well across datasets \cite{Sarode2019PCRNetPC}.  Finally, we show registration results on KITTI and Apollo.

Figure~\ref{fig:best_buddy_pairs} shows the best-buddies pairs during a typical softBBS run on the Stanford Bunny model~\cite{Turk:1994:ZPM}. The algorithm converges after 120 iterations. At first, there are few best-buddies pairs, but as time progresses their number grows until convergence. We also inspected the evolution of the matrix ${\bar B}$ over time (not shown). We observed that the matrix is nearly binary throughout the optimization process, which indicates that our soft approximation is quite close to the sharp best-buddies similarity $B$.

\iffalse
\paragraph{{\bf Accuracy and Basin of Convergence Trade-Off.}}

Next, we try to evaluate the accuracy and basin of convergence of softBBS, softBD, and softBDN. To illustrate these properties, we sampled all three loss functions at different angles around the ground-truth angle (Figure~\ref{fig:BBS_BD_BDN}). The setup is as follows: we used a down-sampled version of the Bunny model with 200 points. We rotated the target point cloud in a known angle, shown as the GT angle in the figure, and for simplicity did not apply any translation. We then measured the values of the three loss functions, in different angles around the GT angle. As can be seen, the subplots have different Y-axis values. This is related to the different characteristics of the losses - while softBBS is an approximation of the hardBBS, that equals to negative the number of the best-buddy pairs, softBD and softBDN should approximate the average distances of the best-buddy pairs (point-to-point and point-to-plane distances, respectively).  All three variants have local minimum around the GT angle. SoftBBS has the largest basin of convergence, allowing to smoothly perform gradient descent from a wide range of starting angles. However, softBBS did not reach minimum exactly at the GT angle. SoftBD and softBDN have steeper slopes, which may indicate their ability to convergence accurately. They both reached minimum at the desired angle. Experiments in Section \ref{subsec:Accuracy} further show that softBDN provides better accuracy compared to softBD.
 
 \begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{BBS_BD_BDN2.png} 
    \caption{{\bf Accuracy vs. Basin of Convergence:} SoftBBS (top), softBD (middle) and softBDN (bottom) loss functions, sampled around the GT angle. As can be seen, softBBS has the largest basin of convergence, while softBD and softBDN are more accurate. Combining the three gives us a flexible algorithm with a large basin of convergence and high accuracy.}
    \label{fig:BBS_BD_BDN}
\end{figure}

\fi


\subsection{Performance Evaluation Setup}
\label{subsec:PerformanceEvaluation}

We conduct a set of experiments to evaluate accuracy
%, basin of convergence, as well as 
and robustness to measurement noise and distractors. To do that, we apply different rotations, translations, sub-sampling, and noise, to each point cloud. Then we compare ourselves to the following popular point cloud registration algorithms: (i) HGMR~\cite{Eckart_2018_ECCV}, a GMM based method; (ii) Coherent Point Drift (CPD)~\cite{Myronenko:2010:PSR}, a probabilistic algorithm based on GMM; (iii) FilterReg (FReg)~\cite{FilterReg}, a probabilistic point-set registration algorithm; and (iv) Symmetric ICP  (Sym-ICP)~\cite{Rusinkiewicz:2019:ASO}, which provides state-of-the-art performances on several point cloud registration challenges. 

ICP algorithms are sensitive to noise, and therefore commonly employ a set of standard practices for outlier rejection. SoftBBS and softBD require no such process. In softBDN, we follow~\cite{Rusinkiewicz:2019:ASO} and remove points whose distance is greater than $3$ times the standard deviation of distances (\cite{Rusinkiewicz:2019:ASO} uses a factor of $2.5$). Notice that Sym-ICP uses additional filtering strategies, such as eliminating points with negative normals dot product, which is not required for our method. 

\paragraph{\bf{Setting.}} We use few variants of our approach in different settings. We denote by \emph{BBR} a version where we first optimize on the softBBS loss, and then refine the result by the softBD loss. In both cases, the distance measure is the Euclidean point-to-point distance. \emph{BD} denotes a version where we only optimize on the softBD loss, and is typically used in experiments where the initial error is not very large. \emph{BDN} uses the \emph{BD} loss with the symmetric point-to-plane distance measure that uses normals (Equation~\eqref{eq:normals}). Normals are estimated for all points in the point cloud (before sub-sampling), by calculating the principal axis of a neighborhood of $k=13$ neighbors around each point. For consistency, Sym-ICP was given the same normals used for \emph{BDN}. In all variants, the optimization is performed by running Adam for a pre-defined number of iterations. 

%\paragraph{\bf{Accuracy.}}
\subsection{Accuracy}
\label{subsec:Accuracy}

The experiments shown in Figure~\ref{fig:accuracy} demonstrate the ability of \emph{BD} and \emph{BDN} to register point clouds with random rotation and translation, using the Bunny, Horse, and Dragon point clouds from~\cite{Turk:1994:ZPM}.
We randomly select a source and target subset from the original point cloud, each containing $M$ points. The target point cloud is rotated around a randomly selected axis by an angle of $\theta_{rot}$. It is then translated along a random axis to a distance of $\Delta_{trans}$. We then run all the registration algorithms on the point-cloud pair and record their translational and rotational error. We repeat the experiment $T$ times and report the median error for each algorithm and each cardinality $M$ of the point clouds.

\begin{figure}[t]
    \centering
    \hspace*{0.5cm}\includegraphics[width=2.5cm]{accuracy_bun_back_vis.png}
    \hspace*{1cm}\includegraphics[width=3cm]{accuracy_horse_visualization.png}
    \hspace*{1cm}\includegraphics[width=3cm]{accuracy_dragon_visualization.png}\\
    \includegraphics[width=3.9cm]{accuracy_bunny_rotation.png} 
    \includegraphics[width=4cm]{accuracy_horse_rotation.png}
    \includegraphics[width=4.05cm]{accuracy_dragon_rotation.png} \\
    \includegraphics[width=3.9cm]{accuracy_bunny_translation.png} 
    \includegraphics[width=4cm]{accuracy_horse_translation.png}
    \includegraphics[width=4.05cm]{accuracy_dragon_translation.png}
     \caption{{\bf Accuracy test:} Top - Point clouds examples as used in the accuracy test. The Bunny (left) is down-sampled to 1000 points, and rotated by 8 degrees. The Horse (middle) is rotated by 10 degrees, and contains only 200 points. The Dragon (right) is rotated by 5 degrees and has 2000 points. Bottom - angular and translation error as a function of the number of points. \emph{BDN} achieves the most accurate results in all scenarios.} 
    \label{fig:accuracy}
\end{figure}

For all experiments in Figure~\ref{fig:accuracy} we set $\Delta_{trans}\!=\!0.005$ meters and $T\!=\!20$. The experiment on the left uses the Bunny point cloud, with $M\in\{200,300,\ldots,1000\}$, and $\theta_{rot}\!=\!8$ degrees. For the Horse point cloud in the middle, we use the same range of $M$ values, and $\theta_{rot}\!=\!10$ degrees. Finally for the Dragon model on the right, we generated point clouds with higher point density, of up to $M\!=\!2000$, and use $\theta_{rot}\!=\!5$ degrees. We see that the \emph{BDN} version of our method achieves lower error rate, across all point cloud sizes, than any of the other methods. Only when the point density is high, Sym-ICP performs on-par with \emph{BDN}. We should also notice that \emph{BD} outperforms any registration method that does not use normals. In the Horse experiment, we omitted FReg~\cite{FilterReg} results, which were inferior to the other methods.


\subsection{\bf{Robustness}}
\label{subsec:ExperimentsRobustness}
The next experiment demonstrates the resistance of the algorithm to a variety of challenges, including occlusions, the presence of a distractor, measurement noise, and a large initial error.

\paragraph{{\bf Partial Overlap and Occlusion.}}
\label{subsec:RobustnessPartialBun}
The experiment shown in Figure~\ref{fig:PartialBun} evaluates the resistance to partial overlap and occlusion. We perform registration between two partial scans of the Stanford Bunny, \emph{bun000} and \emph{bun090}, each captured from a different view point. Following Rusinkiewicz's \cite{Rusinkiewicz:2019:ASO} experimental setup, we first align the scans according to the ground truth motion. Then we follow the same experimental method as in Section~\ref{subsec:Accuracy}, with $M\in\{200,300,\ldots,1000\}$, $\theta_{rot}\!=\!5$ degrees and $\Delta_{trans}\!=\!0.005$ meters. We compare our \emph{BD} and \emph{BDN} algorithms with Sym-ICP \cite{Rusinkiewicz:2019:ASO}. \emph{BDN} achieves the most accurate results, though generally all three algorithms handle the challenge well. However, Sym-ICP deteriorates considerably when given a very sparse point cloud, while both of our algorithms cope with it very well.

\begin{figure}[t]
    \includegraphics[width=4.8cm]{partialbun_rob_rotation.png}
    \includegraphics[width=5cm]{partialbun_rob_translation.png}
    \includegraphics[width=2cm]{parital_bunny_rob_aligned_distractor_visualization.png} 
    \caption{{{\bf{Robustness to point of view changes:}} Right - aligned \emph{bun000} and \emph{bun090} with 1000 points, with overlap of less than 30\%. Left - angular and translation error for varying number of points. both \emph{BDN} and \emph{BD} outperform Sym-ICP \cite{Rusinkiewicz:2019:ASO} when the number of samples is low.}}
    \label{fig:PartialBun}
\end{figure}

\paragraph{\bf{Resistance to Distractors.}}
This experiment evaluates the effects of distractor noise. This is the case where in addition to the main object of interest, the scene also contains a second object with a different motion. In this synthetic experiment, the main object - the Horse, was randomly translated and rotated as in Section~\ref{subsec:Accuracy}, with $M\!=\!1000$, $T\!=\!20$, $\theta_{max}\!=\!10$ degrees and $\Delta_{trans}\!=\!0.005$ meters. The position of the distractor object was randomized across the scene. In Figure~\ref{fig:Distractor_noise} we show the median error as a function of the strength of the noise, defined as the fraction of the points in the point cloud that belong to the distractor. \emph{BD} and \emph{BDN} are able to achieve low errors even for very high levels of noise, where the other algorithms fail. 


\begin{figure}[t]
    \centering
    \includegraphics[width=4.8cm]{distractor_rotation.png}
    \includegraphics[width=5cm]{distractor_translation.png}
    \includegraphics[width=2.2cm]{distractor_visualization.png}
    \caption{{\bf Distractor noise:} Right - an example of our experimental setting, where 40\% of the points belong to the distractor object. Left - the angular and translation error for varying distractor strengths. Both \emph{BD} and \emph{BDN} are not affected by the presence of the distractor, as long as the majority of points belong to the main object. They also achieve the lowest errors for high levels of noise, indicating their robustness.}
    \label{fig:Distractor_noise}
\end{figure}


\paragraph{\bf{Measurement noise.}}
The TUM RGB-D dataset \cite{DBLP:conf/iros/SturmEEBC12} contains point clouds of indoor scenes captured with the Kinect sensor. It contains natural measurement noise, due to the warp and scanning noise from the Kinect sensor. It has been noted by Rusinkiewicz \cite{Rusinkiewicz:2019:ASO} that this dataset poses a qualitatively different challenge than the bunny point cloud. He demonstrates his algorithm on a specific pair of partially-overlapping scans from this dataset. We use the same pair, 1305031104.030279 and 1305031108.503548 of the {freiburg1\_xyz} sequence from the TUM RGB-D (Figure ~\ref{fig:TUM_images}), sample 1000 points from each, and experiment with adding a random rotation of up to $5$ degrees around a random axis. We repeat this 50 times and perform registration for each, showing the cumulative distribution of the final errors in Figure~\ref{fig:TUM}. BBR performs considerably better than either Sym-ICP~\cite{Rusinkiewicz:2019:ASO} or CPD~\cite{Myronenko:2010:PSR}, showing its robustness to realistic measurement noise and occlusions. 

\begin{figure}[t]
    \centering
    \includegraphics[width=5cm]{RGB-D.png}
    \includegraphics[width=3cm]{tum.png}
    \begin{tabular}{cc}
    \end{tabular}
     \caption{{\bf TUM-RGB-D:} Left - RGB-D image from the TUM-RGBD data set \cite{DBLP:conf/iros/SturmEEBC12}. This data is captured by the Kinect sensor, and exhibits warp and scanning noise. Right - Sampled point clouds of 1000 points of the same scene, emphasizing the small area of overlap.}
     \label{fig:TUM_images}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{tum_ROC.png}
    \caption{{\bf Convergence Analysis (TUM):} The cumulative distribution of errors over $50$ repeats. $x$-axis: the error threshold; $y$ axis: the fraction of results that achieved an error smaller than this threshold. For example, CPD~\cite{Myronenko:2010:PSR} has $0\%$ of its registration results with an error lower than $0.1m$, while Sym-ICP~\cite{Rusinkiewicz:2019:ASO} has $30\%$, and BBR (ours) has $\sim$$100\%$ of its errors lower than this threshold.}
    \label{fig:TUM}
\end{figure}


\paragraph{\bf Large initial error.}
In this experiment we evaluate \emph{BBR}'s ability to converge when starting from a large initial error, meaning the ground-truth motion between the source and target point cloud is large. We use two scans of the bunny point cloud, \emph{bun180} and \emph{bun270}, that were captured from significantly different view points. As before, we first align them, sample 1000 points from each, and then apply a random motion to one of them. In this experiment the motion is large: a random rotation in the range $[30,50]$ degrees, around a random axis, and a translation of half the extent of the point cloud ($0.05$ meters) along a random direction. Figure~\ref{fig:ConvergencePartialBun} shows the cumulative distribution of errors over 50 repeats. \emph{BBR} achieves overall lower errors than either Sym-ICP~\cite{Rusinkiewicz:2019:ASO} or CPD~\cite{Myronenko:2010:PSR}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=8cm]{bun_ROC.png}
    \includegraphics[width=3cm]{partial_bunny_unified.png}
    \caption{{\bf Convergence Analysis (partially-overlapping Bunny):} Right: \emph{bun180} and \emph{bun270}, aligned (top), and in their initial position: rotated in 50 degrees and translated by a factor of 0.05 meters (bottom). Left: the cumulative distribution of errors over $50$ repeats. The $x$-axis is the error threshold and the $y$ axis is fraction of registration results whose error is smaller than this threshold. }
    \begin{tabular}{cc}
    \end{tabular}
    \label{fig:ConvergencePartialBun}
\end{figure}




\begin{table}[t]
	%	\footnotesize
	\small
	\begin{center}
		\begin{tabular}{|p{4.0cm}|cc|cc|}
			\toprule[1pt]
			%Method & \makecell[tc]{Mean Ang. \\ Error($^\circ$)} & \makecell[tc]{Max Ang. \\ Error($^\circ$)} & \makecell[tc]{Mean Trans. \\ Error($m$)} & \makecell[tc]{Max Trans. \\ Error($m$)}  \\
			%\multirow{2}{*}{\makecell[tl]{Method}} &\multicolumn{2}{c}{Angular Error($^\circ$)} &\multicolumn{2}{c}{Translation Error($m$)}  \\
			\multirow{2}{*}{\makecell[tl]{Method}} & Angular & Error($^\circ$) & Translation & Error(m) \\
			\cline{2-3}\cline{4-5}
			& Mean & Max & Mean & Max  \\
			\midrule[.5pt]
			% ICP \cite{ICP}                   & 0.125 & 1.273  & 0.065  & 0.478   \\
			% G-ICP \cite{SegalHT09}               & 0.067 & 0.375  & 0.059  & 0.461   \\
			% AA-ICP \cite{Pavlov2018}             & 0.152 & 1.449  & 0.090  & 1.166   \\
			% NDT-P2D \cite{journals/ijrr/Stoyanov0AL12}             & 0.541 & 9.448  & 0.229  & 2.987   \\
			% GMM-REG \cite{Jian2011}              & 1.959 & 3.901  & 0.776  & 1.485   \\
			% CPD \cite{Myronenko:2010:PSR}             & 0.368 & 2.013  & 0.090  & 2.246   \\
			ICP-Po2Po \cite{ICP}                   & 0.139 & 1.176  & 0.089  & 2.017   \\
			ICP-Po2Pl \cite{ICP}                   & 0.084 & 1.693  & 0.065  & 2.050   \\
			G-ICP \cite{SegalHT09}               & 0.067 & 0.375  & 0.065  & 2.045   \\
			AA-ICP \cite{Pavlov2018}             & 0.145 & 1.406  & 0.088  & 2.020   \\
			NDT-P2D \cite{journals/ijrr/Stoyanov0AL12}             & 0.101 & 4.369  & 0.071  & 2.000   \\
			%GMM-REG \cite{Jian2011}              & 1.879 & 4.865  & 0.778  & 1.544   \\
			CPD \cite{Myronenko:2010:PSR}             & 0.461 & 5.076  & 0.804  & 7.301   \\
			%PPFNet\cite{ppfnet_2018}         & 0.335  & 1.336  & 0.131   & 1.336   \\  
			3DFeat-Net \cite{yew20183dfeat}            & 0.199 & 2.428  & 0.116  & 4.972   \\
			DeepVCP-Base \cite{Lu_2019_ICCV}                               & 0.195  & 1.700  & 0.073   & \textbf{0.482}   \\
			DeepVCP-Duplication  \cite{Lu_2019_ICCV}                                & 0.164  & 1.212  & 0.071  & \textbf{0.482}   \\
			Sym-ICP \cite{Rusinkiewicz:2019:ASO} & 0.066  & 0.422  & \textbf{0.058}   & 0.863   \\
			\midrule[.5pt]
			LBDN (ours)         & \textbf{0.065}  & \textbf{0.356}  & \textbf{0.058}   & 0.730   \\
			%\midrule[.5pt]
			%Ours-Base                                & 0.439  & 2.711  & 0.084   & 0.903   \\
			%Ours-Duplication                                & 0.267  & 1.709  & 0.074  & 0.905   \\
			\bottomrule[1pt] 
		\end{tabular}
	\end{center}
	\vspace{-0.2cm}
	\caption{
		The KITTI Odometry dataset. Our algorithm achieves state of the art results for almost all accuracy measures. 
	}
	\label{tab:kitti}
	\vspace{-0.4cm}
\end{table}

\begin{table}[t]
	%	\footnotesize
	\small
	\begin{center}
		\begin{tabular}{|p{4.0cm}|cc|cc|}
			\toprule[1pt]
			%Method & \makecell[tc]{Mean Ang. \\ Error($^\circ$)} & \makecell[tc]{Max Ang. \\ Error($^\circ$)} & \makecell[tc]{Mean Trans. \\ Error($m$)} & \makecell[tc]{Max Trans. \\ Error($m$)}  \\
			%\multirow{2}{*}{\makecell[tl]{Method}} &\multicolumn{2}{c}{Angular Error($^\circ$)} &\multicolumn{2}{c}{Translation Error($m$)}  \\
			\multirow{2}{*}{\makecell[tl]{Method}} & Angular & Error($^\circ$) & Translation & Error(m) \\
			\cline{2-3}\cline{4-5}
			& Mean & Max & Mean & Max  \\
			\midrule[.5pt]
			% ICP \cite{ICP}                   & 0.035 & 0.586  & 0.052  & 5.236   \\
			% G-ICP \cite{SegalHT09}               & 0.025 & 1.010  & 0.031  & 1.545   \\
			% AA-ICP \cite{Pavlov2018}             & 0.336 & 175.503  & 0.125  & 6.348   \\
			% NDT-P2D \cite{journals/ijrr/Stoyanov0AL12}             & 0.143 & 30.639  & 0.218  & 5.344   \\
			% GMM-REG \cite{Jian2011}              & 1.953 & 39.203  & 0.756  & 1.452   \\
			% CPD \cite{Myronenko:2010:PSR}             & 0.360 & 44.310  & 0.221  & 13.025   \\
			ICP-Po2Po \cite{ICP}                   & 0.051 & 0.678  & 0.089  & 3.298   \\
			ICP-Po2Pl \cite{ICP}                   & 0.026 & 0.543  & 0.024  & 4.448   \\
			G-ICP \cite{SegalHT09}               & 0.025 & 0.562  & 0.014  & 1.540   \\
			AA-ICP \cite{Pavlov2018}             & 0.054 & 1.087  & 0.109  & 5.243   \\
			NDT-P2D \cite{journals/ijrr/Stoyanov0AL12}             & 0.045 & 1.762  & 0.045  & 1.778   \\
			%GMM-REG \cite{Jian2011}              & 1.909 & 3.535  & 0.765  & 1.531   \\
			CPD \cite{Myronenko:2010:PSR}             & 0.054 & 1.177  & 0.210  & 5.578   \\
			%PPFNet \cite{ppfnet_2018}         & 0.240  & 1.507  & 0.088   & 2.979   \\  
			3DFeat-Net \cite{yew20183dfeat}             & 0.076 & 1.180  & 0.061  & 6.492   \\
			DeepVCP-Base \cite{Lu_2019_ICCV}                                & 0.135  & 1.882  & 0.024   & \textbf{0.875}   \\
			DeepVCP-Duplication \cite{Lu_2019_ICCV}                                & 0.056  & 0.875  & 0.018   & 0.932  \\
            Sym-ICP \cite{Rusinkiewicz:2019:ASO} & 0.018  & 2.589  & 0.010   & 6.625   \\
			\midrule[.5pt]			
			LBDN (ours)                                & \textbf{0.015}  & \textbf{0.308}  & \textbf{0.007}   & 2.517  \\			
			% \midrule[.5pt]
			% Ours-Base                                & 0.203  & 2.056  & 0.036   & 1.080   \\
			% Ours-Duplication                                & 0.077  & 0.9191  & 0.026  & 1.055   \\
			\bottomrule[1pt] 
		\end{tabular}
	\end{center}
	\vspace{-0.2cm}
	\caption{
		The Apollo-SouthBay odometry dataset. Our algorithm achieves state of the art results for almost all accuracy measures.  
	}
	\label{tab:apollo}
	\vspace{-0.2cm}
\end{table}

\subsection{Odometry}
\label{subsec:Odometry}

In this section we present experiments in the realistic setting of vehicle navigation, specifically focusing on a difficult setting where the separation between the two clouds is relatively large, leading to significant occlusions and outliers caused by independently moving objects in the scene. We use two datasets of high-resolution Lidar scans: KITTI Odometry~\cite{Geiger2012CVPR}, and Apollo-Southbay~\cite{apollo}, both of which  consist of large point clouds of over 100K points. We follow the experimental setup of~\cite{Lu_2019_ICCV}, where the test set consists of pairs of clouds scanned by the same vehicle at two times, during which the vehicle has travelled up to 5 meters, for up to 2 seconds (KITTI) or even 5 seconds (Apollo-Southbay). An initial estimate for the motion is assumed to be available, which is inaccurate by up to 1 meter in each of x,y,z, and up to 1 degree in each of $\theta, \phi, \psi$. We report the mean translation and angular errors, as well as the maximum (worst case). 


For this test, we use the LBDN variant of our BBR algorithm. Normals are estimated from neighborhoods of $k=94$ points in the full cloud. To achieve high accuracy, we only moderately subsample the point clouds to 30K points, uniformly at random. 


Tables~\ref{tab:kitti} and ~\ref{tab:apollo} compare our results to those reported in~\cite{Lu_2019_ICCV}, and to those of Sym-ICP~\cite{Rusinkiewicz:2019:ASO}. For both experiment, we achieve state of the art accuracy by three of the four accuracy measures. This demonstrates BBR's capabilities of achieving high accuracy in realistic scenarios that include occlusions, outlier motions and measurement noise.

\subsection{Run-time}

Table~\ref{tab:BBR_time} shows the time it takes to run a single iteration of the different variants of our loss function, as a function of the number of points (measured with a PyTorch implementation running on a GM204GL Tesla M60 GPU). All of the algorithm variants typically converge in few hundreds of iterations, depending on the learning rate. 
 
\begin{table}[h]
\begin{center}

\begin{tabular}{|c|c|c|}
\hline
\# Points & \emph{BBS}/\emph{BD} Avg. Iter. Time [msec] & \emph{BDN} Avg. Iter. Time [msec] \\
\hline
200         &                  2     &       2.5           \\
400         &                  8     &       12         \\
800         &                 10     &       20         \\
1000        &                 12     &       25           \\		
\hline
\end{tabular}
\caption{Running time of a single iteration, as a function of the number of points}
\label{tab:BBR_time}
\end{center}
\end{table}
